LOCO: Rethinking Objects for Network Memory

In this work, we explore an object-based programming model for filling the space between shared memory and distributed systems programming. We argue that the natural representation for resources distributed across a memory network (e.g. RDMA or CXL) is the traditional shared memory object. This concurrent object (which we call a "channel" object) exports traditional methods, but, especially in an incoherent or uncacheable memory network, stores its state in a distributed fashion across all participating nodes. In a sense, the channel object's state is stored "across the network". Based on this philosophy, we introduce the Library of Channel Objects (LOCO), a library for building multi-node objects on RDMA. Channel objects are composable and designed for both the strong locality effects and the weak consistency of RDMA. Unlike prior work, channel objects do not hide memory complexity, instead relying on the programmer to use NUMA-like techniques to explicitly manage each object. As a consequence, our channel objects have performance similar to custom RDMA systems (e.g. distributed maps), but with a far simpler programming model. Our distributed map channel has better read and comparable write performance to a state-of-the-art custom RDMA solution, using well-encapsulated and reusable primitives.

==> libpaper-shim.tex <==
% A shim for NVSL's libpaper for when you don't want to use it but are using 
% text that expects it

\usepackage{letltxmacro}
\usepackage{caption}

% These are common enough to get protected

\ifdefined\ignore
\else
\newcommand{\ignore}[1]{}
\fi

\ifdefined\boldparagraph
\else
\newcommand{\boldparagraph}[1]{\vspace*{1ex}\noindent\textbf{#1}\hspace{1em}}
\fi

\newcommand{\noindentparagraph}{\vspace*{1ex}\noindent}

%%%% Saman defs


\usepackage[usenames]{color}
\usepackage{xcolor}


\newcommand{\XP}{Optane}
\newcommand{\Optane}{Optane}
\newcommand{\XPDIMM}{\Optane{} DIMM}
\newcommand{\XPDIMMs}{\Optane{} DIMMs}
\newcommand{\lattest}{LATTester}

\newcommand{\aepline}{OptaneLine}
\newcommand{\APC}{OptaneController}
\newcommand{\RMW}{OptaneBuffer}
\newcommand{\iMC}{iMC}

\newcommand{\hooks}{NVHooks}
\newcommand{\Pname}{\hooks}
\newcommand{\PMEM}{PMem}
\newcommand{\NVMShort}{NVM}
\newcommand{\NVM}{\NVMShort}
\newcommand{\NVMLong}{non-volatile memory}
\newcommand{\DCPMEM}{Intel DC Persistent Memory}

% Evaluation
\newcommand{\MaxOptOverNaive}{27}
\newcommand{\MaxOptOverHCtree}{104}
\newcommand{\MaxOptOverHChash}{97}
\newcommand{\MaxImprovementForInsertsUsingExtraTracking}{119}
\newcommand{\MaxImprovementForLoopCoalescingATLAS}{32}
\newcommand{\MaxImprovementForLoopCoalescingKAMINO}{39}
\newcommand{\MaxImprovementForLoopCoalescingPMDK}{8}
\newcommand{\MaxImprovementForStaticCheck}{5}
\newcommand{\MaxImprovementForFieldCoalescing}{17}
\newcommand{\BptreePMDKOverKamino}{3}
\newcommand{\BptreePMDKOverAtlas}{2}
\newcommand{\HashmapPMDKOverKamino}{8}
\newcommand{\HashmapPMDKOverAtlas}{2}

\newcommand{\cmark}{Yes}
\newcommand{\xmark}{No}


\newcommand{\MM}{}
\newcommand{\PM}{}

\newcommand{\MMLDRAM}{\MM{}DRAM}
\newcommand{\MMPMEMC}{\MM{}Optane-Cached}
\newcommand{\MMPMEMUC}{\MM{}Optane-Uncached}

\newcommand{\PMLDRAM}{\PM{}DRAM}
\newcommand{\PMRDRAM}{\PM{}DRAM-Remote}
\newcommand{\PMLPMEM}{\PM{}Optane}
\newcommand{\PMLPMEMUI}{\PM{}Optane-NI}
\newcommand{\PMRPMEM}{\PM{}Optane-Remote}
%\newcommand{\PMPMEP}{PMEP}


\newcommand{\SSDOptane}{SSD-Optane}
\newcommand{\SSDSATA}{SSD-SATA}

\newcommand{\emusize}{80}

\newcommand{\appdax}{App Direct}

\newcommand{\KernelVersion}{4.13.0}
\newcommand{\aeppersocketsizegb}{1536}
\newcommand{\aeppersocketsizetb}{1.5}
\newcommand{\aepdimmsizegb}{256}
\newcommand{\aeptotalsizetb}{3}
\newcommand{\drampersocketsizegb}{192}
\newcommand{\aepfirmware}{01.01.00.5253}

\newcommand{\OneLM}{App Direct}
\newcommand{\TwoLM}{Memory}
\newcommand{\Emu}{DRAM Emulation}
\newcommand{\OneLMNI}{App Direct Not Interleaved}
\newcommand{\ewrlong}{effective write ratio}
\newcommand{\Ewrlong}{Effective Write Ratio}
\newcommand{\ewr}{EWR}
\newcommand{\ewrfull}{\Ewrlong (\ewr)}

%\newcommand{\black}[1]{\textit{\textbf{\noindent{\underline{#1}}}}}
\newcommand{\black}[1]{\boldparagraph{#1}}

% avoid triggering texlint :(
\newcommand{\timez}[1]{$\times$}

% \newcommand{\pcode}[1]{\texttt{#1}}

\definecolor{lightBlue}{RGB}{189,215,231}
\colorlet{light-orange}{lightBlue!65}
%\lstset{basicstyle={\small\ttfamily},language=C,keywordstyle={\bfseries \color{blue}},morekeywords={size\_t,uintptr\_t,bool}}

\newcommand{\ccode}[1]{
\lstinputlisting[basicstyle={\footnotesize\ttfamily},
    columns=fullflexible,
    escapechar=!,
    firstnumber=last,
    frame=bt,
    framexleftmargin={1em},
    language=C,
    breaklines=true,
    keywordstyle={\bfseries \color{blue}},
    morekeywords={size\_t,uintptr\_t,bool,uint32\_t},
    numbers=left,
    numberstyle={\tiny},
    tabsize=2,
    numbersep=1em,
    xleftmargin=1.5em,
    commentstyle=\color{green},
    literate={*}{{$^{*}$}}1
]{#1}
}

%\newcommand{\markcode}[1]{\colorbox{light-orange}{\strut #1}}
\newcommand{\markcode}[1]{\colorbox{light-orange}{#1}}



%%%% defs

\usepackage{xcolor}

\definecolor{cyanish}{rgb}{0,0.8,1.0}
\definecolor{orange}{rgb}{1.0,0.5,0.0}
\definecolor{pink}{rgb}{1.0,0.47,0.6}
\definecolor{light-gray}{gray}{0.95}
\definecolor{jiancolor}{RGB}{0,153,153}
\definecolor{mygreen}{RGB}{50,200,50}
\definecolor{pink}{rgb}{1.0,0.47,0.6}

\definecolor{commentgreen}{rgb}{0.0,0.5,0.0}


\newcommand{\BigOmega}[1]{$\Omega(#1)$}
\newcommand{\BigO}[1]{${\cal O}(#1)$}
\newcommand{\BigTheta}[1]{$\Theta(#1)$}

\newcommand{\Caveatdaxor}{\emph{Caveat DAXor}}

\newcommand{\DAXmmapd}{DAX-mapped}
\newcommand{\DAXmmap}{DAX-\mmap{}}

\newcommand{\caveatdaxor}{\emph{caveat DAXor}}
\newcommand{\etal}{\textit{et al.}}


\newcommand{\mmapd}{\mmap{}'d} 
\newcommand{\mm}{mm$^2$}
\newcommand{\myitem}[1]{\item \textbf{#1}}% ignore macros
\newcommand{\refalg}[1]{Algorithm~\ref{#1}}% ignore macros
\newcommand{\refeq}[1]{(Equation~\ref{#1})}% ignore macros
\newcommand{\reffig}[1]{Figure~\ref{#1}}% ignore macros
\newcommand{\reflst}[1]{Listing~\ref{#1}}% ignore macros
\newcommand{\refsec}[1]{Section~\ref{#1}}% ignore macros
\newcommand{\reftab}[1]{Table~\ref{#1}}% ignore macros
\newcommand{\refapp}[1]{Appendix~\ref{#1}}% ignore macros
\newcommand{\us}{$\mu$s}
\newcommand{\x}[1]{$\times$}
\newcommand{\figtitle}[1]{\textbf{#1}}


\newcommand{\note}[2]{\fixme{$\ll$ #1 $\gg$ #2}}

\newcommand{\app}[1]{{\sc #1}}

\newcommand{\nova}[1]{NOVA} % ignore macros
\newcommand{\extfs}[1]{\texttt{Ext4#1}}% ignore macros
\newcommand{\extfsDAX}[1]{\extfs{-DAX#1}}% ignore macros
\newcommand{\xfs}[1]{\texttt{XFS#1}}% ignore macros
\newcommand{\xfsDAX}[1]{\xfs{-DAX#1}}% ignore macros
\newcommand{\csym}[1]{\texttt{#1}}% ignore macros

% mbox prevents linebreaks between the name and the '()'
\newcommand{\cfunc}[1]{\mbox{\csym{#1}\hspace{-0.1em}\csym{()}}}% ignore macros

\newcommand{\malloc}{\cfunc{malloc}}% ignore macros
\newcommand{\free}{\cfunc{free}}% ignore macros
\newcommand{\iowrite}{\cfunc{write}}% ignore macros
\newcommand{\ioread}{\cfunc{read}}% ignore macros
\newcommand{\ioctl}{\cfunc{ioctl}}% ignore macros
\newcommand{\mmap}{\cfunc{mmap}}% ignore macros
\newcommand{\munmap}{\cfunc{munmap}}% ignore macros
\newcommand{\fsync}{\cfunc{fsync}}% ignore macros
\newcommand{\msync}{\cfunc{msync}}% ignore macros
\newcommand{\fdatasync}{\cfunc{fdatasync}}% ignore macros
\newcommand{\memcpy}{\cfunc{memcpy}}% ignore macros
\newcommand{\memset}{\cfunc{memset}}% ignore macros
\newcommand{\pread}{\cfunc{pread}}% ignore macros
\newcommand{\pwrite}{\cfunc{pwrite}}% ignore macros
\newcommand{\writev}{\cfunc{writev}}% ignore macros
\newcommand{\readv}{\cfunc{readv}}% ignore macros
\newcommand{\pwritev}{\cfunc{pwritev}}% ignore macros
\newcommand{\preadv}{\cfunc{preadv}}% ignore macros


\newcommand{\eg}{e.g.}


%%%%% SINGLE FIGURE
\def\nfigure[#1,#2,#3]{
\begin{figure}
\vspace*{0mm}
\begin{center}

\includegraphics[width=\columnwidth]{#1} 
\vspace*{-6mm}\caption[]{#2
} \label{#3}

\vspace*{-3mm}
\end{center}
%\horizbar
%\vspace*{-2mm}
\end{figure}}

%%%%% SINGLE FIGURE
\def\cfigure[#1,#2,#3]{
\begin{figure}
\vspace*{0mm}
\begin{center}

\includegraphics[width=3in]{#1} 
\vspace*{-3mm}\caption[]{#2
} \label{#3}
 
\vspace*{-5mm}
\end{center}
%\horizbar
%\vspace*{-2mm}
\end{figure}}

%%%%% SINGLE FIGURE 4in wide
\def\cfigurefour[#1,#2,#3]{
\begin{figure}
\vspace*{0mm}
\begin{center}

\includegraphics[width=4in]{#1} 
\vspace*{-3mm}\caption[]{#2
} \label{#3}
 
\vspace*{-5mm}
\end{center}
%\horizbar
%\vspace*{-2mm}
\end{figure}}

%%%%% SINGLE FIGURE
\def\cfiguretemp[#1,#2,#3]{
\begin{figure}
\vspace*{0mm}
\begin{center}

\includegraphics[width=3.5in]{#1} 
\vspace*{-3mm}\caption[]{#2
} \label{#3}
 
\vspace*{-5mm}
\end{center}
%\horizbar
\vspace*{-2mm}
\end{figure}}

%%%%% SINGLE WIDE FIGURE
\def\wfigure[#1,#2,#3]{
\begin{figure*}
\vspace*{0mm}
\begin{center}
 \includegraphics[width=\textwidth]{#1} 
 \vspace*{-3mm}\caption[]{#2
} \label{#3}
 
\end{center}
%\horizbar
\end{figure*}}

%%%%% 3 FIGURES IN A ROW
\def\threefigure[#1,#2,#3,#4,#5]{
\begin{figure*}
\vspace*{0mm}
\begin{center}

\begin{tabular}{ccc}
\includegraphics[width=2in]{#1} & \includegraphics[width=2in]{#2} &  \includegraphics[width=2in]{#3} \\
(a) & (b) & (c) \\
\end{tabular}
\vspace*{-3mm}\caption[]{#4
} \label{#5}

\vspace*{-5mm}
\end{center}
%\horizbar
\vspace*{-2mm}
\end{figure*}}

%%%%%% DOUBLE FIGURE
\def\dcfigure[#1,#2,#3,#4,#5,#6]{
{
\begin{figure*}
\begin{center}
\begin{minipage}[c]{\columnwidth}{
\includegraphics[width=\columnwidth]{#1} 
\vspace*{0mm}\caption[]{#2} \label{#3} \
}\end{minipage}\hspace*{\columnsep}\
\begin{minipage}[c]{\columnwidth}{
\includegraphics[width=\columnwidth]{#4} 
\vspace*{0mm}\caption[]{#5}\label{#6} \
}\end{minipage}
\end{center}
\end{figure*}
}
}

\def\scfigure[#1,#2,#3]{
{
\begin{figure*}
\begin{center}
\begin{minipage}[c]{3.5in}{
\includegraphics[width=3.5in]{#1} 
}\end{minipage}
\caption[]{#2} \label{#3} \
\end{center}
\end{figure*}
}
}


\def\tableByTable[#1,#2,#3,#4,#5,#6]{
{
\begin{table*}
\begin{center}
\begin{minipage}[c]{3in}{
\centering
{#1}
\vspace*{0mm}\tabcaption[]{#2}\label{#3} \
}\end{minipage}\hspace*{\columnsep}\
\begin{minipage}[c]{3in}{
\centering
{#4}
\vspace*{0mm}\tabcaption[]{#5}\label{#6} \
}\end{minipage}
\end{center}
\end{table*}
}
}


\def\figureByTable[#1,#2,#3,#4,#5,#6]{
{
\begin{figure*}
\begin{center}
\begin{minipage}[c]{3in}{
\centering
\includegraphics[width=\textwidth]{#1}
\vspace*{0mm}\figcaption[]{#2} \label{#3} \
}\end{minipage}\hspace*{\columnsep}\
\begin{minipage}[c]{3.3in}{
\centering
{#4}
\vspace*{0mm}\tabcaption[]{#5}\label{#6} \
}\end{minipage}
\end{center}
\end{figure*}
}
}

\def\tableByFigure[#1,#2,#3,#4,#5,#6]{
{
\begin{figure*}
\begin{center}
\begin{minipage}[c]{4.3in}{
\centering
{#1}
\vspace*{0mm}\tabcaption[]{#2} \label{#3} \
}\end{minipage}\hspace*{\columnsep}\
\begin{minipage}[c]{2.2in}{
\centering
\includegraphics[width=\textwidth]{#4}
\vspace*{-0.35in}\caption[]{#5}\label{#6} \
}\end{minipage}
\end{center}
\end{figure*}
}
}

% two figs pdfs in one column fig
\def\doublecfigure[#1,#2,#3,#4]{
{
\begin{figure}
\begin{center}
\begin{minipage}[c]{1.5in}{
\begin{center}
\includegraphics[width=1.5in]{#1}%\\(a)
\end{center}
}\end{minipage}\hspace*{1em}\
\begin{minipage}[c]{1.5in}{
\begin{center}
\includegraphics[width=1.5in]{#2}%\\(b)
\end{center}
}\end{minipage}
\vspace*{0mm}\caption[]{#3} \label{#4} \
\end{center}
\end{figure}
}
}

\def\qcfigure[#1,#2,#3,#4,#5,#6]{
{
\begin{figure*}
\vspace*{0.2in}\
\begin{center}
\begin{minipage}[c]{3in}{
\includegraphics[width=3in]{#1} 
\vspace*{-3mm}
}
\end{minipage}\hspace*{0.5in}\
\begin{minipage}[c]{3in}{
\includegraphics[width=3in]{#2} 
\vspace*{-3mm}
}\end{minipage}

\begin{minipage}[c]{3in}{
\includegraphics[width=3in]{#3} 
\vspace*{-3mm}
}
\end{minipage}\hspace*{0.5in}\
\begin{minipage}[c]{3in}{
\includegraphics[width=3in]{#4} 
\vspace*{-3mm}
}\end{minipage}
\end{center}
\caption[]{#5}\label{#6}
\end{figure*}
}
}

\def\twfigure[#1,#2,#3,#4,#5]{
{
\begin{figure*}
\vspace*{0.2in}\
\begin{center}
\begin{minipage}[c]{6.5in}{
\includegraphics[width=6.5in]{#1} 
\vspace*{-3mm}
}
\end{minipage}

\begin{minipage}[c]{6.5in}{
\includegraphics[width=6.5in]{#2} 
\vspace*{-3mm}
}\end{minipage}

\begin{minipage}[c]{6.5in}{
\includegraphics[width=6.5in]{#3} 
\vspace*{-3mm}
}
\end{minipage}
\end{center}
\caption[]{#4}\label{#5}
\end{figure*}
}
}

\def\dwfigure[#1,#2,#3,#4]{
{
\begin{figure*}
\vspace*{0.2in}\
\begin{center}
\begin{minipage}[c]{6.5in}{
\includegraphics[width=6.5in]{#1} 
\vspace*{-3mm}
}
\end{minipage}

\begin{minipage}[c]{6.5in}{
\includegraphics[width=6.5in]{#2} 
\vspace*{-3mm}
}\end{minipage}

\end{center}
\caption[]{#3}\label{#4}
\end{figure*}
}
}



\def\dssfigure[#1,#2,#3,#4,#5,#6]{
{
\begin{figure*}
\vspace*{0.2in}\
\begin{center}
\begin{minipage}[c]{4in}{
\includegraphics[width=4in]{#1}
\vspace*{-3mm}\caption[]{#2} \label{#3} \
}\end{minipage}\hspace*{0.5in}\
\begin{minipage}[c]{2in}{
\includegraphics[width=2in]{#4}
\vspace*{-3mm}\caption[]{#5}\label{#6} \
}\end{minipage}
\end{center}
\vspace*{-0.4in}\
\end{figure*}
}
}




\def\dsfigure[#1,#2,#3,#4,#5,#6]{
{
\begin{figure*}
\vspace*{0.2in}\
\begin{center}
\begin{minipage}[c]{3in}{
\includegraphics[width=3in]{#1}
\vspace*{-3mm}\caption[]{#2} \label{#3} \
}\end{minipage}\hspace*{0.5in}\
\begin{minipage}[c]{3in}{
\hspace*{0.5in}\
\includegraphics[height=3in]{#4}
\vspace*{-3mm}\caption[]{#5}\label{#6} \
}\end{minipage}
\end{center}
\vspace*{-0.4in}\
\end{figure*}
}
}


\def\dsyfigure[#1,#2,#3,#4,#5,#6]{
{
\begin{figure*}
\vspace*{0.2in}\
\begin{center}
\begin{minipage}[c]{2.5in}{
\includegraphics[height=2.5in]{#1}
\vspace*{-3mm}\caption[]{#2} \label{#3} \
}\end{minipage}\hspace*{0.5in}\
\begin{minipage}[c]{2.5in}{
\includegraphics[height=2.5in]{#4}
\vspace*{-3mm}\caption[]{#5}\label{#6} \
}\end{minipage}
\end{center}
\vspace*{-0.4in}\
\end{figure*}
}
}

\def\dyfigure[#1,#2,#3,#4,#5,#6]{
{
\begin{figure*}
\vspace*{0.2in}\
\begin{center}
\begin{minipage}[c]{3in}{
\includegraphics[height=3in]{#1} 
\vspace*{-3mm}\caption[]{#2} \label{#3} \
}\end{minipage}\hspace*{0.5in}\
\begin{minipage}[c]{3in}{
\includegraphics[height=3in]{#4} 
\vspace*{-3mm}\caption[]{#5}\label{#6} \
}\end{minipage}
\end{center}
\vspace*{-0.4in}\
\end{figure*}
}
}

%%%%%% DOUBLE FIGURE Y
\def\dyoldfigure[#1,#2,#3,#4,#5,#6]{
{
\begin{figure*}
\vspace*{0.2in}\
\begin{center}
\begin{minipage}[c]{3in}{
\epsfysize=2.0in\
\hspace{0.5in}\
\epsfbox{#1}
\vspace*{-3mm}\caption[]{#2} \label{#3} \
}\end{minipage}\hspace*{0.25in}\
\begin{minipage}[c]{3in}{
\epsfysize=2.0in\
\hspace{0.5in}\
\epsfbox{#4}
\vspace*{-3mm}\caption[]{#5}\label{#6} \
}\end{minipage}
\end{center}
\vspace*{-0.4in}\
\end{figure*}
}
}

%%%%%% DOUBLE FIGURE Y IN A COLUMN!!
\def\cfiguredouble[#1,#2,#3,#4]{
\begin{figure}
\vspace*{0.2in}\
\begin{center}
\begin{minipage}[c]{1.5in}{
\epsfxsize=1.5in\
\epsfbox{#1}
}\end{minipage}\hspace*{0.1in}\
\begin{minipage}[c]{1.5in}{
\epsfxsize=1.5in\
\vspace{0.1in}\epsfbox{#2}
}\end{minipage}\vspace*{-0.10in} \caption[]{#3}\label{#4}
\end{center}
\vspace*{-0.4in}\
\end{figure}
}


%%%%% Single programmable size figure
\def\wpfigure[#1,#2,#3,#4]{
\begin{figure*}
\vspace*{4mm}
\begin{center}

\includegraphics[width=#4]{#1} 

\vspace*{-3mm}\caption[]{#2
} \label{#3}

\vspace*{-5mm}
\end{center}
%\horizbar
\end{figure*}}

%%%%% Single programmable size figure, rotated
\def\wprfigure[#1,#2,#3,#4,#5]{
\begin{figure*}
\vspace*{4mm}
\begin{center}

\includegraphics[width=#4, angle=#5]{#1} 

\vspace*{-3mm}\caption[]{#2
} \label{#3}

\vspace*{-5mm}
\end{center}
%\horizbar
\end{figure*}}




%%%%% Adjacent, programmable-width figures, slid vertically by 9th
%%%%% parameter
\def\DoubleFigureWSlide[#1,#2,#3,#4,#5,#6,#7,#8,#9]{
\begin{figure*}
\vspace*{#9}
\begin{center}
\begin{minipage}{#4}
\includegraphics[width=#4]{#1}
\vspace*{-3mm}\caption{#2
}\label{#3}
\end{minipage}
\hspace{2em}
\begin{minipage}{#8}
\includegraphics[width=#8]{#5}
\vspace*{-3mm}\caption{#6
}\label{#7}
\end{minipage}
\vspace*{-5mm}
\end{center}
\end{figure*}
}


%%%%% Adjacent, programmable-width figures
\def\DoubleFigureW[#1,#2,#3,#4,#5,#6,#7,#8]{
\begin{figure*}
\vspace*{0in}
\begin{center}
\begin{minipage}{#4}
\includegraphics[width=#4]{#1}
\vspace*{-3mm}\caption{#2
}\label{#3}
\end{minipage}
\hspace{2em}
\begin{minipage}{#8}
\includegraphics[width=#8]{#5}
\vspace*{-3mm}\caption{#6
}\label{#7}
\end{minipage}
\vspace*{-5mm}
\end{center}
\end{figure*}
}



\def\DoubleFigureWHack[#1,#2,#3,#4,#5,#6,#7,#8]{
\begin{figure*}
\vspace*{0in}
\begin{center}
\begin{minipage}{3in}
\includegraphics[width=#4]{#1}
\vspace*{-3mm}\caption{#2
}\label{#3}
\end{minipage}
\hspace{2em}
\begin{minipage}{3in}
\includegraphics[width=#8]{#5}
\vspace*{-3mm}\caption{#6
}\label{#7}
\end{minipage}
\vspace*{-5mm}
\end{center}
\end{figure*}
}






%%%%%% DOUBLE FIGURE
\def\ddcfigure[#1,#2,#3,#4]{
\begin{figure*}
\vspace*{0.2in}\
\begin{center}
\begin{minipage}[c]{\columnwidth}{
\includegraphics[width=\columnwidth]{#1} 
}\end{minipage}\hspace{0.5in}\
\begin{minipage}[c]{\columnwidth}{
\includegraphics[width=\columnwidth]{#2} 
}\end{minipage} \caption[]{#3}\label{#4}
\end{center}
\end{figure*}
}

\def\ddcfigureSlide[#1,#2,#3,#4,#5]{
\begin{figure*}
\vspace*{#5}\
\begin{center}
\begin{minipage}[c]{3in}{
\includegraphics[height=3in]{#1} 
}\end{minipage}\hspace{0.5in}\
\begin{minipage}[c]{3in}{
\includegraphics[height=3in]{#2} 
}\end{minipage}\vspace*{-0.10in} \caption[]{#3}\label{#4}
\end{center}
\vspace*{-0.4in}\
\end{figure*}
}

\def\cxfigure[#1,#2,#3]{
\begin{figure}
\vspace*{4mm}
\begin{center}
 
\epsfxsize=2.5in\
\epsfbox{#1}\
 
\vspace*{-0.10in}\caption[]{#2
} \label{#3}
 
\vspace*{-5mm}
\end{center}
%\horizbar
\vspace*{-2mm}
\end{figure}}

\newenvironment{panefigure}{\begin{figure}\begin{center}}{\end{center}\end{figure}}

\newcommand{\pdfpane}[3]{
\begin{minipage}{#1}
\begin{center}
\includegraphics[width=#1]{#2}\\(#3)
\end{center}
\end{minipage}
}




==> relwork.tex <==
\section{Related Work}
\label{sec:relwork}


Given the issues with the existing network memory programming model, many works
have sought to propose alternatives. We divide these
into two categories: disaggregated container models, and distributed 
shared memory models.
We also discuss other applications of the RDMA protocol.

\subsection{Disaggregated Containers}

The works most related to LOCO are those which encapsulate network memory
operations in distributed container objects.

BCL~\cite{brock-icpp-2019} describes an infrastructure for developing containers
using network memory through parallel programming libraries such as
MPI~\cite{bonachea-lcpc-2019} or GASNet~\cite{graham-ppam-2006}, and implements
some containers using this infrastructure.  Unlike LOCO, the BCL backend relies
on a flat global address space provided by the underlying parallel programming
library. In addition, BCL containers are neither reusable nor composable.
Finally, the BCL backend and containers divide participants into clients and
servers, while LOCO treats all peers equally on the backend, but allows the
implementation of client-server designs as asymmetric channel endpoints.

HCL~\cite{devarajan-cluster-2020} builds on BCL. 
HCL inherits the flat address space and client-server
model of BCL, and still relies on MPI for setup. However, unlike BCL containers,
the memory regions underlying HCL containers have unique names, allowing reuse.
Unlike LOCO channels, the containers are not composable and have a less flexible
relationship with memory: each HCL container is associated with exactly one
local memory region on each node.

Quicksand~\cite{ruan-hotos-2023} provides sharded data containers which aim to
efficiently manage disaggregated resources using the ``proclet'' model
introduced in Nu~\cite{ruan-nsdi-2023}. Quicksand focuses on the management of
disaggregated resources in the backend, which is orthogonal to LOCO's focus on
the application programming model; its insights could likely be integrated into
LOCO without significant changes to this model.

Finally, Outside the Box~\cite{aguilera-hotos-2019} proposes extensions to the
RDMA protocol, along with new container designs based on these extensions. The
work is focused on the details of the container algorithms, rather than the
structure of the object system. We expect that the proposed extensions and data
structures could be easily supported in LOCO.

\subsection{Flattening the Address Space}

A second, much larger, body of work presents a unified view of network memory to
the application as a single coherent address space in a shared memory abstraction, 
either with purely
software-based virtualization~\cite{gouk-atc-2022, cai-vldb-2018,
wang-osdi-2020, zhang-sigmod-2022, ruan-osdi-2020}, or by extending
hardware~\cite{calciu-asplos-2021}. These works generally focus on transparently
(or mostly-transparently~\cite{ruan-osdi-2020, zhang-sigmod-2022}) porting
existing shared memory applications, while LOCO provides a clean-slate approach
based on encapsulating communication in objects. Additionally, LOCO differs
in making local and remote memory semantically distinct, as
the programmer must treat them differently for maximum
performance.

However, there is a good deal of work on caching or pooling systems which
improve the performance of a flat, coherent address space on network
memory~\cite{feng-osdi-2023, maruf-asplos-2023, li-asplos-2023, shen-sosp-2023,
wang-nsdi-2023, guo-sosp-2023}, and it is plausible that these innovations could
tip the tradeoff between performance and the ease-of-use provided by coherence
to favor the latter in some cases. Even so, these systems must themselves be
implemented on a backend which distinguishes local and remote memory, and we
argue that LOCO is a strong contender to be that backend.

\subsection{RDMA Applications}

RDMA has found many uses in the application space due to its
strong performance. It has been used to accelerate 
consensus~\cite{aguilera-osdi-2020,izraelevitz-icpp-2022,jha-tocs-2019,
poke-hpdc-2015, aguilera-podc-2019}, distributed transaction
processing~\cite{dragojevic-sosp-2015}, distributed
databases~\cite{barthels-sigmod-2015}, distributed key-value
stores~\cite{wang-sigmod-2022, dragojevic-nsdi-2014, li-fast-2023,
kalia-sigcomm-2014}, replicated key-value stores~\cite{alquraan-nsdi-2024}, \cite{gavrielatos-ppopp-2020}, 
graph processing~\cite{wang-jpdc-2023}, and distributed
learning~\cite{xue-eurosys-2019, ren-hpcc-2017}. Other work explores extensions
to RDMA NIC support~\cite{burke-sosp-2021}, reusable optimization
techniques~\cite{ma-cluster-2021}, or the overlap between persistence and
RDMA~\cite{yang-fast-2019, yang-nsdi-2020, zhang-fast-2022}. Broadly,
integrating RDMA into applications is useful when the
major performance bottleneck is communication delay.


